Tensor-Algebraic Property Skeletons: Guiding Agents to Construct Semantic Oracles for DL Compilers

Deep learning (DL) compilers optimize tensor computation graphs through transformations that can silently change what a model computes. Existing work generates well-formed computation graphs and tensor inputs but typically judges results through crashes or differential comparison. Tensor algebra offers stronger oracles, such as commutativity and reduction decomposition, but turning an identity into an executable check requires selecting applicable operators, valid inputs, and precision-aware comparisons. We present Propilot, an agentic testing framework that guides LLM agents to construct semantic oracles from tensor algebra. Its core abstraction, the property skeleton, couples a relation with applicability conditions and an oracle template whose compiler-specific slots the agent fills. Propilot comes with sixteen skeletons and twenty data generators. It validates each test before execution and uses rejection reasons, execution results, and usage records to steer generation toward untested combinations. We evaluate Propilot with six agents on three DL compilers against Agent-Only, which uses the same agents without Propilot. Propilot detects 96 distinct compiler root causes, including 25 with silent wrong outputs that Agent-Only misses. It also generates 85.34% fewer invalid tests and covers at least 2.73 times as many operator-property pairs on each compiler. On 161 faulty TVM versions, Propilot detects 100, against 53 for Agent-Only.

==> figures/eval-style.tex <==
\definecolor{evalPropilot}{HTML}{0072B2}
\definecolor{evalAgent}{HTML}{E69F00}
\definecolor{evalCrash}{HTML}{56B4E9}
\definecolor{evalRepaired}{HTML}{A66A00}
\definecolor{evalInk}{HTML}{1F2328}
\definecolor{evalAxis}{HTML}{8A949E}
\definecolor{evalGrid}{HTML}{E4E8EC}
\pgfplotsset{compat=1.16}
\ifdefined\evalPatternsDeclared\else
\pgfdeclarepatternformonly{evalNE}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{6pt}{6pt}}{\pgfqpoint{5pt}{5pt}}{%
  \pgfsetlinewidth{0.5pt}\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}\pgfpathlineto{\pgfqpoint{5.1pt}{5.1pt}}\pgfusepath{stroke}}
\pgfdeclarepatternformonly{evalNW}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{6pt}{6pt}}{\pgfqpoint{5pt}{5pt}}{%
  \pgfsetlinewidth{0.5pt}\pgfpathmoveto{\pgfqpoint{0pt}{5pt}}\pgfpathlineto{\pgfqpoint{5.1pt}{-0.1pt}}\pgfusepath{stroke}}
\gdef\evalPatternsDeclared{}
\fi
\pgfplotsset{
  eval base/.style={
    font=\sffamily\footnotesize,
    /pgf/number format/assume math mode=true,
    tick label style={font=\sffamily\footnotesize, text=evalInk},
    label style={font=\sffamily\footnotesize, text=evalInk},
    title style={font=\sffamily\footnotesize\bfseries, text=evalInk},
    axis x line*=bottom, axis y line*=left,
    axis line style={evalAxis, line width=0.5pt},
    major tick style={evalAxis, line width=0.5pt},
    major tick length=2pt,
    ymajorgrids, grid style={evalGrid, line width=0.4pt},
    scaled ticks=false,
    legend cell align=left,
    legend style={draw=none, fill=none, font=\sffamily\footnotesize, text=evalInk,
                  /tikz/every even column/.append style={column sep=9pt}},
  },
  eval bars/.style={
    eval base, ybar,
    legend image code/.code={\fill[#1, draw=none] (0cm,-0.075cm) rectangle (0.34cm,0.125cm);},
    x tick style={draw=none}, xtick pos=bottom,
    nodes near coords, nodes near coords align={vertical},
    nodes near coords style={font=\sffamily\scriptsize, text=evalInk, fill=white,
                             inner sep=0.7pt, yshift=0.6pt},
  },
  eval bar/.style={draw=none, fill=#1},
  eval texture/.style={postaction={pattern=#1, pattern color=white, fill opacity=0.85}},
  eval lines/.style={
    eval base, scale only axis, width=108pt, height=47pt, clip=false,
    xmin=0, xmax=24.65, xtick={0,6,12,18,24},
    tick label style={font=\sffamily\scriptsize, text=evalInk},
    title style={yshift=-3pt, text height=1.6ex, text depth=0.4ex},
  },
  eval prop line/.style={evalPropilot, line width=1.1pt, line join=round},
  eval agent line/.style={evalAgent, line width=1.1pt, line join=round, dash pattern=on 2.8pt off 1.5pt},
  eval prop mark/.style={mark=*, mark size=1.9pt, mark options={solid, fill=evalPropilot, draw=white, line width=0.5pt}},
  eval agent mark/.style={mark=square*, mark size=1.7pt, mark options={solid, fill=evalAgent, draw=white, line width=0.5pt}},
}
\definecolor{evalAgentDark}{HTML}{C48700}
\definecolor{evalAblation}{HTML}{CC79A7}
\pgfdeclareplotmark{evalcell}{\pgfpathrectangle{\pgfpoint{-0.5*\evalcellw}{-0.5*\evalcellh}}{\pgfpoint{\evalcellw}{\evalcellh}}\pgfusepathqfill}
\pgfplotsset{
  keep panel/.style={x filter/.expression={\thisrow{panel}==#1 ? x : nan}},
  keep compiler/.style={x filter/.expression={\thisrow{compiler_index}==#1 ? x : nan}},
  eval curves/.style={
    eval base, scale only axis, clip=false, xmin=0, xmax=6, xtick={0,2,4,6}, ymin=0,
    tick label style={font=\sffamily\fontsize{6}{7}\selectfont, text=evalInk},
    label style={font=\sffamily\scriptsize, text=evalInk},
    title style={yshift=-3pt, font=\sffamily\scriptsize\bfseries, text=evalInk},
    ylabel style={yshift=-3pt},
  },
  eval coverage/.style={
    eval base, scale only axis, clip=true, y dir=reverse, xtick=\empty, ymajorgrids=false, axis y line*=none, axis x line*=none, axis line style={black!45, line width=0.3pt},
    tick label style={font=\sffamily\fontsize{5.2}{5.6}\selectfont, text=evalInk}, major tick length=0pt, yticklabel style={inner sep=1.5pt},
    label style={font=\sffamily\scriptsize, text=evalInk}, title style={yshift=-3pt, font=\sffamily\scriptsize\bfseries, text=evalInk},
    ylabel style={font=\sffamily\scriptsize\bfseries, yshift=-2pt}, xlabel style={yshift=3pt, font=\sffamily\fontsize{6}{7}\selectfont},
  },
  eval cell/.style={only marks, mark=evalcell, mark options={fill=#1, draw=none}, color=#1},
  eval validity bars/.style={
    eval base, xbar, scale only axis, width=112pt, height=62pt, clip=false, xmin=0, xmax=128, xtick={0,50,100},
    ymin=0.45, ymax=3.55, ytick={1,2,3}, ymajorgrids=false, xmajorgrids, y tick style={draw=none}, bar width=8pt,
    tick label style={font=\sffamily\fontsize{6.5}{7.5}\selectfont, text=evalInk},
    label style={font=\sffamily\scriptsize, text=evalInk}, title style={yshift=-3pt, font=\sffamily\scriptsize\bfseries, text=evalInk},
    nodes near coords={\pgfmathprintnumber[fixed, fixed zerofill, precision=2]{\pgfplotspointmeta}}, point meta=x,
    nodes near coords style={font=\sffamily\fontsize{6}{7}\selectfont, text=evalInk, inner sep=1.2pt, anchor=west, fill=none},
    every node near coord/.append style={xshift=0pt},
  },
}
\tikzset{
  eval prop series/.style={evalPropilot, line width=1pt, line join=round},
  eval agent series/.style={evalAgentDark, line width=0.8pt, line join=round, dash pattern=on 2.4pt off 1.2pt},
  eval opus/.style={solid},
  eval gpt61/.style={dash pattern=on 3pt off 1.4pt},
  eval gpt55/.style={dash pattern=on 0.9pt off 1.1pt},
  eval noskeleton/.style={evalAblation, line width=0.8pt, line join=round, dash pattern=on 3pt off 1.4pt},
  eval novalidation/.style={black!60, line width=0.8pt, line join=round, dash pattern=on 0.9pt off 1.1pt},
  eval nofeedback/.style={evalAblation!65!black, line width=0.8pt, line join=round, dash pattern=on 3.4pt off 1.1pt on 0.8pt off 1.1pt},
  eval wrong/.style={fill=evalPropilot, draw=evalInk, line width=0.35pt},
  eval crash/.style={pattern=crosshatch, pattern color=evalInk, draw=evalInk, line width=0.35pt},
  eval internal/.style={pattern=north east lines, pattern color=evalInk, draw=evalInk, line width=0.35pt},
  eval exception/.style={fill=white, draw=evalInk, line width=0.35pt},
}
\tikzset{
  eval leader/.style={draw=black!35, line width=0.25pt},
  eval end label/.style={anchor=west, inner sep=0pt, font=\sffamily\scriptsize, text=evalInk},
  eval row label/.style={anchor=west, align=left, inner sep=0pt, font=\sffamily\footnotesize, text=evalInk},
  eval axis label/.style={anchor=north, inner sep=0pt, font=\sffamily\footnotesize, text=evalInk},
}

